Efficient Binary Decision Diagram Manipulation in External Memory

We follow up on the idea of Lars Arge to rephrase the Reduce and Apply procedures of Binary Decision Diagrams (BDDs) as iterative I/O-efficient algorithms. We identify multiple avenues to simplify and improve the performance of his proposed algorithms. Furthermore, we extend the technique to other common BDD operations, many of which are not derivable using Apply operations alone, and we provide asymptotic improvements for the procedures that can be derived using Apply. These algorithms are implemented in a new BDD package, named Adiar. We see very promising results when comparing the performance of Adiar with conventional BDD packages that use recursive depth-first algorithms. For instances larger than 8.2 GiB, our algorithms, in parts using the disk, are 1.47 to 3.69 times slower compared to CUDD and Sylvan, exclusively using main memory. Yet, our proposed techniques are able to obtain this performance at a fraction of the main memory needed by conventional BDD packages to function. Furthermore, with Adiar we are able to manipulate BDDs that outgrow main memory and so surpass the limits of other BDD packages.

==> data/io_buddy_tic_tac_toe_21_time.tex <==
4  38.264
5  37.099
6  37.144
7  37.783
8  1536.349
9  2448.810
10 2975.066


==> data/memory_15_queens_adiar_time.tex <==
2   5498.039
4   5080.602
8   4685.659
12  4611.500
16  4518.153
20  4419.179
26  4353.587
32  4252.071
48  4067.247
56  3970.994
64  3962.365
72  3974.343
80  3981.235
96  3931.487
128 3988.846
192 4004.051
256 3952.037


==> data/memory_15_queens_cudd_time.tex <==
72  3023.328
80  2980.696
96  2783.778
128 2883.858
192 2646.368
256 2507.809


==> data/memory_15_queens_sylvan_time.tex <==
56  2076.672
64  2075.058
72  2073.201
80  2075.893
96  1985.152
128 1876.851
192 1874.785
256 1884.510


==> data/memory_N_queens_adiar_time_per_node.tex <==
7 14.4425648718522
8 6.27786067996692
9 2.59706239564784
10 1.10300483461721
11 0.542048344231203
12 0.40070067193074
13 0.418284029735695
14 0.443586359689405
15 0.810577629867117


==> data/queens_adiar_time.tex <==
% 7  8.001
% 8  8.667
% 9  9.718
% 10 10.094
% 11 14.727
12 31.373
13 123.567
14 662.924
15 3970.070
16 31017.033
17 267296.390

==> data/queens_adiar_time_per_node.tex <==
12 1.2222
13 1.0156
14 1.0362
15 1.0635
16 1.3654
17 1.8352


==> data/queens_buddy_time.tex <==
12 4.117
13 23.255
14 142.423

==> data/queens_buddy_time_per_node.tex <==
12 0.17650
13 0.19865
14 0.22357

==> data/queens_cudd_time.tex <==
12 8.967
13 52.881
14 316.093
15 2687.585


==> data/queens_cudd_time_per_node.tex <==
12 0.38433
13 0.45169
14 0.49618
15 0.72473


==> data/queens_sylvan_time.tex <==
12 7.160
13 45.805
14 309.479
15 1860.749


==> data/queens_sylvan_time_per_node.tex <==
12 0.30688
13 0.39125
14 0.48580
15 0.49530


==> data/tic_tac_toe_adiar_time.tex <==
20 29.513
21 124.148
22 599.800
23 2815.244
24 12479.837
25 43574.274
26 104621.760
27 234606.020
28 478232.065
29 772581.531


==> data/tic_tac_toe_adiar_time_per_node.tex <==
20 1.166372461896
21 0.924212677039
22 0.922490241336
23 1.012835952731
24 1.238317630089
25 1.452515906095
26 1.442743291417
27 1.63443822957
28 2.015663720143
29 2.300389983801


==> data/tic_tac_toe_buddy_time.tex <==
20 4.032
21 23.371
22 128.102
23 667.436


==> data/tic_tac_toe_buddy_time_per_node.tex <==
20 0.159347195011
21 0.17398407123
22 0.197020414964
23 0.24012241104


==> data/tic_tac_toe_cudd_time.tex <==
20 7.626
21 48.172
22 255.093
23 1257.012
24 5246.023


==> data/tic_tac_toe_cudd_time_per_node.tex <==
20 0.301385269611
21 0.358613901141
22 0.392332162389
23 0.452233263576
24 0.520517324283


==> data/tic_tac_toe_sylvan_time.tex <==
20 6.973
21 53.607
22 293.725
23 1386.782
24 5244.662
25 17420.893


==> data/tic_tac_toe_sylvan_time_per_node.tex <==
20 0.276
21 0.399
22 0.452
23 0.499
24 0.520
25 0.581

